Advancing Location-Invariant and Device-Agnostic Motion Activity Recognition on Wearable Devices

Wearable sensors have permeated into people's lives, ushering impactful applications in interactive systems and activity recognition. However, practitioners face significant obstacles when dealing with sensing heterogeneities, requiring custom models for different platforms. In this paper, we conduct a comprehensive evaluation of the generalizability of motion models across sensor locations. Our analysis highlights this challenge and identifies key on-body locations for building location-invariant models that can be integrated on any device. For this, we introduce the largest multi-location activity dataset (N=50, 200 cumulative hours), which we make publicly available. We also present deployable on-device motion models reaching 91.41% frame-level F1-score from a single model irrespective of sensor placements. Lastly, we investigate cross-location data synthesis, aiming to alleviate the laborious data collection tasks by synthesizing data in one location given data from another. These contributions advance our vision of low-barrier, location-invariant activity recognition systems, catalyzing research in HCI and ubiquitous computing.

==> notes.tex <==

%To mitigate these challenges, we propose a set of pre-processing steps and leverage data augmentation to achieve a sampling-rate agnostic system and mitigate the performance degradation across different devices and sensor.

%; too many to effectively solve with merely collecting more data. 


   
 
%With that observation and assuming data collection from various body locations is possible, several questions come to mind: 
% \begin{enumerate}
% % \vspace{-1}
%     \item Can we build a universal motion model that learns a joint representation for classifying motion activities from all possible sensor body locations? 
%     \item Given the challenge in capturing data from every possible location, is there a set of key body locations that captures the full-body motion pattern allowing us to build a universal motion model that can easily transfer to other unseen locations? %that is able to recognize activities from any data irrespective of the body location the sensor is placed on?
%     \item Can we learn a mapping of the motion data from one sensor location to another, thus enabling cross-location data synthesis? 
%     % \vspace{-1}
% \end{enumerate}

% \textcolor{red}{while valuable, limitation is that the source and target are defined. We just want one universal model that works. Assumption is that distribution discrepancy will make it hard for model to learn across all, we show it's possible and define the \textit{EigenLocations} that allow a full-body coverage.} 

% \textcolor{red}{2- Another problem space is the cross-view prediction or recovering missing views? --- Data Synthesis problem}

% \textcolor{red}{3- Temporal Alignment? Motion Matching ? }





% what people have done
% what is our objective
% what did we do



%All these devices equipped with IMU sensors capture the same physical activity from different perspectives. 


% Multiple devices on a user’s body are capturing the same physical phenomenon (i.e., a user’s activity) from different perspectives. For example, when a user is running, both a smartphone placed in the thigh pocket and a smartwatch worn on the wrist record sensor data for the running activity, but from different perspectives due to their unique placements on the body. 



%Visually inspecting the spectrograms of the accelerometer signal across different locations, we can identify the dominant frequencies for a user walking with varying intensity depending on the sensor location. For the sensor placed on the ankle, the dominant frequency has a higher intensity compared to that corresponding to data captured from the wrist or head. This can be mapped to variations in the brightness of an image in computer vision. 

% When analyzing time-series, important information is generally manifested in both time and frequency domains. While Fourier Transform (FT) is one of the most widely used techniques in analyzing the frequency content of a signal, it does not retain important time information. To counter this and represent the signal in a joint time-frequency domain, Short-Time-Fourier-Transform (STFT) can be used. 
